Car that Knows Before You Do: Anticipating Maneuvers via Learning Temporal Driving Models

Advanced Driver Assistance Systems (ADAS) have made driving safer over the last decade. They prepare vehicles for unsafe road conditions and alert drivers if they perform a dangerous maneuver. However, many accidents are unavoidable because by the time drivers are alerted, it is already too late. Anticipating maneuvers beforehand can alert drivers before they perform the maneuver and also give ADAS more time to avoid or prepare for the danger. In this work we anticipate driving maneuvers a few seconds before they occur. For this purpose we equip a car with cameras and a computing device to capture the driving context from both inside and outside of the car. We propose an Autoregressive Input-Output HMM to model the contextual information alongwith the maneuvers. We evaluate our approach on a diverse data set with 1180 miles of natural freeway and city driving and show that we can anticipate maneuvers 3.5 seconds before they occur with over 80\% F1-score in real-time.

==> intro_old.tex <==
% !TEX root = main.tex
\section{Introduction}

Over the last decade
cars have been equipped with various assistive technologies to
provide a safe driving experience. Technologies such as lane keeping, blind spot check,
pre-crash systems etc.,  are successful in alerting drivers whenever they commit a
dangerous maneuver~\citep{Laugier11,Lefevre12}. Still in the US alone more than 33,000 people die in road
accidents every year, the majority of which are due to inappropriate
maneuvers~\cite{road_accidents}. 
Studies show that many such 
accidents can be averted if drivers are alerted of danger \textit{before} the maneuver
occurs~\citep{Rueda04}.  In this work we anticipate maneuvers that a
driver is likely to perform in the next few seconds. We use
various cues from inside and outside of the vehicle (Figure~\ref{fig:intro}), and 
present a learning algorithm for reasoning about the future maneuvers.

Anticipating future human actions have recently gained attention both in
robotics and learning communities~\citep{Kuderer12,Kitani12,Wang13,Koppula13}. 
Anticipating maneuvers requires the contextual information from  surrounding events. In our approach, we equip a car with two cameras and a computing device to extract informative signals such as views of the road and the driver, vehicle dynamics, global position coordinates (GPS), and we augment these informations with the street maps. Our setup provides a time series of multi-modal context from both inside and outside of the vehicle. The challenge lies in modeling the temporal aspects to identify contextual cues that help in anticipating next few seconds of driving. 

For anticipation, joint reasoning of driver's intention and the context from surrounding events is also necessary. Firstly,  it is not clear how the context and intention influence one another. 
For example, the intention is influenced by some events, such as traffic conditions,  and influences other events like driver's own head movements. These interactions between the context and driver's intention give a generative nature to the problem that requires a modeling approach specially tailored  to it. Secondly, the driver's intentions are not observable which further introduce latent factors in the model.
	

\iffalse
Anticipating future human actions have recently gained attention both in
robotics and learning communities~\citep{Kuderer12,Kitani12,Wang13,Koppula13}. 
In this work, we address anticipation for assistive vehicles that could be useful for 
 Advanced Driver Assistance Systems (ADAS) so they can avoid or prepare for unsafe 
 situations on the road \cite{Liebner12,Kumar13}. In order to anticipate maneuvers we need to jointly reason over the space of possible driving actions, 
 the rich information from the surrounding context, various road conditions  (e.g., 
intersections, traffic signals, other vehicles, etc) as well as the driver's \textit{latent} intentions. This makes the problem challenging. 
 

In our approach, we equip a car with two cameras and a computing device to extract informative signals for anticipation while driving. One of the cameras face the driver and other faces the road, and the device extracts vehicle dynamics, global position coordinates (GPS) and augments them with the street maps.
Our setup provides multi-modal context from both inside and outside of the vehicle. 
We reason from several signals including, driver's head movement while
they scan for traffic before the maneuver, the knowledge of
surrounding environment such as vehicle lane information, and road artifacts like intersections, turns or highway exits based on the vehicle's GPS location
and speed. We also take into account the overall route of the car using driver's final destination, if available.
\fi
 
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{../Fig/PlaceHolder_intro}
\caption{\textbf{Anticipating maneuvers.} Shows our algorithm anticipating maneuver few seconds in the future. Based of the driver's face movements, GPS and map information it anticipates with high confidence that the driver is likely to turn left at the approaching intersection.}
\label{fig:intro}
\end{figure}


\iffalse
In our approach we set a car with two cameras, one facing the driver and
other facing the road, and a computing device -- for vehicle dynamics, global position coordinates (GPS) and street maps -- in order to extract informative signals for anticipation.
Our setup provides multi-modal context from both inside and outside of the vehicle. We reason from signals such as, driver's head movement while
they scan for traffic before the maneuver, the knowledge of the
surrounding environment such as vehicle lane information, and road artifacts like intersections, turns or highway exits based on the vehicle's GPS location
and speed. We also take into account the global intent of drivers
such as their final destination, if available. 
\fi

For anticipating maneuvers \textit{several seconds} in advance, we propose a model to  capture the generative behavior of observations from these multiple sources.
Our model is an
Autoregressive Input-Output Hidden Markov (AIO-HMM) that jointly captures the context
from inside and outside of the vehicle.  AIO-HMM models how events from outside the vehicle affect driver's behavior which then generates events inside the vehicle. We learn separate AIO-HMM models for each maneuver and during inference we anticipate the probability of each maneuver. 


We evaluate our approach on 1180 miles of natural freeway and
city driving data set collected across 2 states, from 10 drivers and with different kinds of driving maneuvers.
% such as \textit{left lane change, right lane change, left turn, right turn}, and many instances of \textit{no action} i.e. driving straight. 
We show our approach allows anticipating 
maneuvers 3.5 seconds before they occur with 80\% precision and recall. We
believe our work creates scope for new ADAS features to make roads safer.  
In summary our key contributions are as follows: 
\begin{itemize}
\item We propose an approach for anticipating driving maneuvers several seconds in advance.
%\item We propose an novel approach for anticipating driving maneuvers several seconds in advance.
%This is different from systems that warn after the maneuver has occurred. 
\item We model the rich context from inside and outside the vehicle with an autoregressive input-output HMM. 
%\item We model the rich multi-modal contextual driving information  with an autoregressive input-output HMM. 
%Our model captures three important aspects of driving. 
\item We release the first dataset of natural driving with videos of both inside and
outside the car, GPS, speed information, and with lane and driving maneuver annotations.
%We hope this will allow benchmarking of results. 
\end{itemize}
\iffalse
In particular, we reason over multi-modal cues such as drivers head movement
before they perform the maneuver, the lane information of the car, its speed,
braking pattern and GPS location. We also take into account global intent of
drivers such as their final destination, if available. This combination of
various cues allows us to handle various anticipate maneuvers. For example,
before a maneuver drivers move their head to scan environment head to scan
environment. This reasoning using several context enables us to anticipate
actions maneuvers before they occur. For example, drivers move their head to
scan surrounding before executing maneuver, or the lane in which the car is 


In particular, drivers head movement provide strong cues of their upcoming
maneuver. For example, before lane change or turns drivers scan the surrounding,
similarly they check for crossing traffic before driving through an
intersection. We extract such visual cues from a driver facing dashboard camera.
In addition to the inside context, the context outside enables localizing the
car to indentify space of possible safe maneuvers. For example, the lane in
which the car is restricts the space of safe actions. When in the left-most
lane, further left-lane change is not a safe maneuver. Only safe maneuvers are
right-lane change or keep-straight unless the car reaches an intersection. We
get the lane information from a road facing camera. We use car GPS coordinates
to detect an approaching intersection. Finally we draw priors over maneuvers
from speed of the car. 
\fi


\iffalse 
In this work, we address anticipation for a safety critical assistive driving application, where  
we predict the future driving maneuvers in advance. This is useful for systems such as
 Advanced Driver Assistance Systems (ADAS) to avoid or prepare for unsafe 
 situations on the road \cite{Liebner12,Kumar13}.
 The goal of anticipation is to reason over a person's future actions given their 
previous actions, current state and the surrounding context. 
Anticipating driving maneuvers is extremely challenging as it requires 
joint modeling of the action space and rich information from the surrounding context, 
while reasoning about the various road conditions (e.g., 
intersections, traffic signals, other vehicles, etc) as well as the drivers intentions. 
\fi


\iffalse
Anticipation widens the scope of developing better
assistive technologies by allowing robots to autonomously reason over
how can they assist humans in an ongoing activity~\citep{Koppula13}, or to
plan sociable paths by predicting human trajectories~\citep{Kitani12}. In this
work, we perform anticipation for a safety critical application. Anticipating
maneuvers will also Advanced Driver Assistance Systems (ADAS)
 to avoid or prepare for unsafe situations~\cite{Liebner12,Kumar13}.
 


 Anticipation advances many applications. It allows robots to autonomously
reason on how to assist humans with a task~\citep{Koppula13}, or how to
plan sociable paths by predicting human trajectories~\citep{Kitani12}. In this
work, we perform anticipation for a safety critical application, one that could
potentially save thousands of lives on roads.
\fi

\iffalse
We anticipate maneuvers with the help of multi-modal contextual information
from both inside and outside the vehicle. 
Our approach combines various informative
signals such as, driver's head movement while
they scan the surrounding before the maneuver, the knowledge of the
surrounding environment such as vehicle lane information, whether it's
approaching an intersection, turn or a highway exit based on its GPS location
and speed. We also take into account global intent of drivers
such as their final destination, if available. 
We propose a model to combine information from these multiple sources to predict
maneuvers \textit{several seconds} into the future. Our model is an
Autoregressive Input-Output Hidden Markov (AIO-HMM) that captures the contextual
information in-and-out of the car, and reasons on how they influence drivers
mental state before the maneuver. 
\fi

\iffalse
the mental state of driver along with three important 
aspects of driving: (1) how outside environment affects
the drivers \textit{latent} mental state, (2) how latent mental states produce
observable informative cues such as drivers head movement, and (3) how the 
informative cues can occur at
variable time before the maneuver.
\fi



\iffalse


to combine observations from these multiple sources


We propose a model to combine observations from these multiple sources. The modeling challenge is to accurately capture the generative behaviour of observations  to anticipate
maneuvers \textit{several seconds} into the future.
Our model is an
Autoregressive Input-Output Hidden Markov (AIO-HMM) that jointly captures the contextual
information from inside and outside of the vehicle.  AIO-HMM models how events outside the vehicle affect the drivers behaviour when then generates inside vehicle observations. We learn separate AIO-HMM models for each maneuver and perform inference using dynamic programming. 
\fi

